Efficient Multimodal Learning from Data-centric Perspective

Multimodal Large Language Models (MLLMs) have demonstrated notable capabilities in general visual understanding and reasoning tasks. However, their deployment is hindered by substantial computational costs in both training and inference, limiting accessibility to the broader research and user communities. A straightforward solution is to leverage smaller pre-trained vision and language models, which inevitably cause significant performance drops. In this paper, we demonstrate the possibility of training a smaller but better MLLM with high-quality training data. Specifically, we introduce Bunny, a family of lightweight MLLMs with flexible vision and language backbones for efficient multimodal learning from selected training data. Experiments show that our Bunny-4B/8B outperforms the state-of-the-art large MLLMs on multiple benchmarks. We expect that this work can provide the community with a clean and flexible open-source tool for further research and development. The code, models, and data can be found in https://github.com/BAAI-DCAI/Bunny.

==> figures/demo.tex <==
% \begin{figure}[p]
%     \centering
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc1.jpg}
%         % \caption{Caption for Image 1}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc2.jpg}
%         % \caption{Caption for Image 2}
%     \end{subfigure}

%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc3.jpg}
%         % \caption{Caption for Image 2}
%     \end{subfigure}


    
%     % \caption{Overall caption for the figure.}
%     % \label{fig:demo}
% \end{figure}

% \begin{figure}[p]
%     \centering
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc4.jpg}
%         % \caption{Caption for Image 1}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc5.jpg}
%         % \caption{Caption for Image 2}
%     \end{subfigure}

%     \begin{subfigure}{\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/dc6.jpg}
%         % \caption{Caption for Image 2}
%     \end{subfigure}

%     \caption{\textbf{Qualitative test cases of Bunny}: The bold text represents user input, while the non-bold part is the model response. The results demonstrate Bunny's versatile capabilities in visual understanding, common sense reasoning, external knowledge referring, optical character recognizing, and mathematical problem solving.}
%     \label{fig:demo}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[p]
%     \centering
    
%     % First row
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc1.jpg}
%         % \caption{Caption for Image 1}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc2.jpg}
%         % \caption{Caption for Image 2}
%     \end{subfigure}
    
%     % Second row
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc3.jpg}
%         % \caption{Caption for Image 3}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc4.jpg}
%         % \caption{Caption for Image 4}
%     \end{subfigure}
    
%     % Third row
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc5.jpg}
%         % \caption{Caption for Image 5}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dc6.jpg}
%         % \caption{Caption for Image 6}
%     \end{subfigure}

%     \caption{\textbf{Qualitative test cases of Bunny}: The bold text represents user input, while the non-bold part is the model response. The results demonstrate Bunny's versatile capabilities in visual understanding, common sense reasoning, external knowledge referring, optical character recognizing, and mathematical problem solving.}
%     \label{fig:demo}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[p]
    \centering
    % Image 1
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc1.jpg}
    \end{subfigure}
    
    % Image 2
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc2.jpg}
    \end{subfigure}

        % Image 1
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc1.jpg}
    \end{subfigure}
    
    % Image 2
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc3.jpg}
    \end{subfigure}

        % Image 1
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc5.jpg}
    \end{subfigure}
    
    % Image 2
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/dc6.jpg}
    \end{subfigure}

    \caption{\textbf{Qualitative test cases of Bunny}: The bold text represents user input, while the non-bold part is the model response. The results demonstrate Bunny's versatile capabilities in visual understanding, common sense reasoning, external knowledge referring, optical character recognizing, and mathematical problem solving.}
    \label{fig:demo}
\end{figure}


==> tables/main_result.tex <==
\begin{table}
    % \captionsetup{font=tiny}
    \centering
    \caption{{ Comparison to state-of-the-art MLLMs on 11 benchmarks.} Our model outperforms them in most of the settings. We evaluate these models on benchmarks: MME$^\text{P}$: MME perception \cite{mme}, MME$^\text{C}$: MME cognition \cite{mme}, MMB$^\text{T}$: MMBench \cite{mmbench} test split, MMB$^\text{D}$: MMBench \cite{mmbench} dev split, SEED: SEED-Bench-1 \cite{seedbench}, MMMU$^\text{V}$: MMMU \cite{yue2023mmmu} validation split,  MMMU$^\text{T}$: MMMU \cite{yue2023mmmu} test split, VQA-v2 \cite{goyal2017making} test-dev split, GQA \cite{GQA2019} test-dev-balanced split, SQA$^\text{I}$: ScienceQA-IMG \cite{lu2022learn} test split and POPE \cite{li-etal-2023-evaluating}: the averaged F1-score of three categories (random, popular and adversarial) on the validation set of MSCOCO. We mark the best performance \textbf{bold} and the runner-up \underline{underlined} for models with 7B or smaller LLM backbones. 
    %$^*$The training images of the datasets are observed during training. 
    $^\mathsection$We evaluate the officially released checkpoint by ourselves.}
   \setlength{\tabcolsep}{3pt}
 \resizebox{\textwidth}{!}{%
    %\begin{tabular}{l l | p{8mm}p{8mm}p{8mm}p{8mm}p{8mm} | p{8mm}p{8mm}p{8mm}p{8mm}p{9mm}p{8mm}p{9mm}p{12.5mm}p{8mm} }
        \begin{tabular}{l | ll | ccccccccccc}
            \toprule
            Model & Vision Encoder & LLM & MME$^\text{P}$ & MME$^\text{C}$ & MMB$^\text{T}$ & MMB$^\text{D}$ & SEED & MMMU$^\text{V}$ & MMMU$^\text{T}$ & VQA$^\text{v2}$ & GQA & SQA$^\text{I}$ & POPE \\
            \midrule
            IDEFICS-80B \cite{idefics} & OpenCLIP-H (1.0B) & LLaMA-65B & -- & -- & 54.6 & 54.5 & -- & -- & -- & 60.0 & -- & 68.9 & -- \\
            BLIP-2 \cite{li2023blip} & EVA01-CLIP-G (1.0B) & Vicuna-13B & -- & -- & -- & -- & -- & -- & -- & -- & 41.0 & 61.0 & -- \\
            InstructBLIP \cite{instructblip} & EVA01-CLIP-G (1.0B) & Vicuna-13B & -- & -- & -- & -- & -- & -- & -- & -- & 49.5 & 63.1 & 83.7 \\
            BLIP-2 \cite{li2023blip} & EVA01-CLIP-G (1.0B) & Flan-T5-XXL (11B) & 1293.8 & 290.0 & -- & -- & -- & 35.4 & 34.0 & 65.0 & 44.6 & 64.5 & -- \\
            InstructBLIP \cite{instructblip} & EVA01-CLIP-G (1.0B) & Flan-T5-XXL (11B) & 1212.8 & 291.8 & -- & -- & -- & 35.7 & 33.8 & -- & 47.9 & 70.6 & -- \\
            Shikra-13B \cite{chen2023shikra} & CLIP-L (0.4B)& Vicuna-13B & -- & -- & -- & -- & -- & -- & -- & 77.4 & -- & -- & -- \\
            LLaVA-v1.5-13B (LoRA) \cite{liu2023improvedllava} & CLIP-L (0.4B) & Vicuna-13B & 1541.7 & 300.4$^\mathsection$ & 68.4$^\mathsection$ & 68.5 & 61.3 & 40.0$^\mathsection$ & 33.2$^\mathsection$ & 80.0 & 63.3 & 71.2 & 86.7 \\
            \midrule        
            InstructBLIP \cite{instructblip} & EVA01-CLIP-G (1.0B) & Vicuna-7B & -- & -- & 33.9 & 36.0 & 53.4 & -- & -- & -- & 49.2 & 60.5 & -- \\
            MiniGPT-v2 \cite{chen2023minigptv2} & EVA01-CLIP-G (1.0B) & LLaMA2-7B & -- & -- & -- & -- & -- & -- & -- & -- & 60.3 & -- & -- \\
            IDEFICS-9B \cite{idefics} & OpenCLIP-H (1.0B) & LLaMA-7B & -- & -- & 45.3 & 48.2 & -- & -- & -- & 50.9 & -- & 44.2 & -- \\
            LLaVA-v1.5-7B (LoRA) \cite{liu2023improvedllava} & CLIP-L (0.4B) & Vicuna-7B & \underline{1476.9} & 267.9$^\mathsection$ &  \underline{66.1$^\mathsection$} & 66.1 & \underline{60.1} & 34.4$^\mathsection$ & 31.7$^\mathsection$ & 79.1 & \textbf{63.0} & 68.4 & 86.4 \\
            mPLUG-Owl2 \cite{ye2023mplugowl2} & CLIP-L (0.4B) & LLaMA2-7B & 1450.2 & \textbf{313.2} & 66.0 & 66.5 & 57.8 & 32.7 & \underline{32.1} & 79.4 & 56.1 & 68.7 & 85.8 \\
            Shikra-7B \cite{chen2023shikra} & CLIP-L (0.4B)& Vicuna-7B & -- & -- & 60.2 & 58.8 & -- & -- & -- & -- & -- & -- & -- \\
            TinyGPT-V \cite{yuan2023tinygpt} & EVA01-CLIP-G (1.0B) & Phi-2 (2.7B) & -- & -- & -- & -- & -- & -- & -- & -- & 33.6 & -- & -- \\
            Gemini Nano-2 \cite{team2023gemini} & -- & Gemini Nano-2 (3.25B) & -- & -- & -- & -- & -- & 32.6 & -- & 67.5 & -- & -- & -- \\
            MobileVLM \cite{chu2023mobilevlm} & CLIP-L (0.4B) & MobileLLaMA (2.7B) & 1288.9 & -- & -- & 59.6 & -- & -- & -- & -- & 59.0 & 61.0 & 84.9 \\
            MobileVLM V2 \cite{chu2024mobilevlm} & CLIP-L (0.4B) & MobileLLaMA (2.7B) & 1440.5 & -- & -- & 63.2 & -- & -- & -- & -- & 61.1 & \underline{70.0} & 84.7 \\
            LLaVA-Phi \cite{zhu2024llava} & CLIP-L (0.4B) & Phi-2 (2.7B) & 1335.1 & -- & -- & 59.8 & -- & -- & -- & 71.4 & -- & 68.4 & 85.0 \\
            MC-LLaVA \cite{MC-LLaVA} & SigLIP-SO (0.4B) & Dolphin 2.6 Phi-2 (2.7B) & -- & -- & -- & -- & -- & -- & -- & 64.2 & 49.6 & -- & 80.6 \\
            Imp-v1 \cite{imp2024} & SigLIP-SO (0.4B) & Phi-2 (2.7B) & 1434.0 & -- & -- & 66.5 & -- & -- & -- & \underline{79.5} & 58.6 & \underline{70.0} & \textbf{88.0} \\
            MiniCPM-V \cite{minicpm2024} & SigLIP-SO (0.4B) & MiniCPM (2.7B) & 1446.0 & -- & -- & \underline{67.3} & -- & \underline{34.7} & -- & -- & -- & -- & -- \\
            Moondream1 \cite{moondream1} & SigLIP-SO (0.4B) & Phi-1.5 (1.3B) & -- & -- & -- & -- & -- & -- & -- & 74.3 & 56.3 & -- & -- \\
            TinyLLaVA-v1 \cite{tinyllava} & CLIP-L (0.4B) & TinyLlama (1.1B) & -- & -- & -- & -- & -- & -- & -- & 73.4 & 57.5 & 59.4 & -- \\
            \textbf{Bunny} & SigLIP-SO (0.4B) & Phi-2 (2.7B) & \textbf{1488.8} & \underline{289.3} & \textbf{69.2} & \textbf{68.6} & \textbf{62.5} & \textbf{38.2} & \textbf{33.0} & \textbf{79.8} & \underline{62.5} & \textbf{70.9} & \underline{86.8} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:main}
\end{table}

